GAFusion: Adaptive Fusing LiDAR and Camera with Multiple Guidance for 3D Object Detection

Recent years have witnessed the remarkable progress of 3D multi-modality object detection methods based on the Bird's-Eye-View (BEV) perspective. However, most of them overlook the complementary interaction and guidance between LiDAR and camera. In this work, we propose a novel multi-modality 3D objection detection method, named GAFusion, with LiDAR-guided global interaction and adaptive fusion. Specifically, we introduce sparse depth guidance (SDG) and LiDAR occupancy guidance (LOG) to generate 3D features with sufficient depth information. In the following, LiDAR-guided adaptive fusion transformer (LGAFT) is developed to adaptively enhance the interaction of different modal BEV features from a global perspective. Meanwhile, additional downsampling with sparse height compression and multi-scale dual-path transformer (MSDPT) are designed to enlarge the receptive fields of different modal features. Finally, a temporal fusion module is introduced to aggregate features from previous frames. GAFusion achieves state-of-the-art 3D object detection results with 73.6$\%$ mAP and 74.9$\%$ NDS on the nuScenes test set.

==> table/Study_LGAFT.tex <==
\begin{table}
  \centering
  \begin{adjustbox}{width=0.32\textwidth}
  \begin{tabular}{lccll}
    \toprule
    & {Methods} & {LGAFT} & {mAP$\uparrow$} & {NDS$\uparrow$}   \\
\midrule
& BEVFusion & & 70.2  & 72.9 \\
& BEVFusion & \checkmark & 71.0\textcolor[rgb]{0,0.5,0}{$_{\uparrow 0.8}$}  & 73.4\textcolor[rgb]{0,0.5,0}{$_{\uparrow 0.5}$}  \\
\hdashline
& MSMDFusion & & 71.5  & 74.0 \\
& MSMDFusion & \checkmark & 72.1\textcolor[rgb]{0,0.5,0}{$_{\uparrow 0.6}$}  & 74.3\textcolor[rgb]{0,0.5,0}{$_{\uparrow 0.3}$} \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{Generalization of LGAFT module on the nuScenes dataset.}\vspace{-0.2cm}
  \label{tab:study_LGAFT}
\end{table}

==> table/waymo_count.tex <==
\begin{table}
  \centering
  \begin{adjustbox}{width=0.3\textwidth}
  \begin{tabular}{@{}lccccc@{}}
    \toprule
    & {Class} & {3D obeject} & {2D object}   \\
\midrule
& Vehicle & 6.1M  & 9.0M \\
& Pedestrian & 2.8M  & 2.7M  \\
& Cyclist & 67k  & 81k \\
& Sign & 3.2M  & - \\
    \bottomrule
  \end{tabular}
  \end{adjustbox}
  \caption{The number of 3D and 2D objects of different categories on the Waymo dataset.}\vspace{-0.2cm}
  \label{tab:wamyo_count}
\end{table}

==> table/waymo_test_result.tex <==
\begin{table}
  \centering
  \begin{adjustbox}{width=0.47\textwidth}
  \begin{tabular}{l|c|cccc}
    \hline
         Methods & Modality & AP/L1 & APH/L1 & AP/L2 & APH/L2 \\
    \hline
    PV-RCNN++ & L & 80.26 & 78.71 & 75.00 & 73.52\\
    MPPNet & L & 81.83 & 80.59 & 76.88 & 75.67\\
    CenterFormer & L & 82.26 & 80.91 & 77.60 & 76.29 \\
   
    \hline
    DeepFusion & LC & 81.90 & 80.48  & 76.91 & 75.54\\
    BEVFusion & LC & 82.72 & 81.35 & 77.65 & 76.33 \\
    % LoGoNet~\cite{yan2023cmt} & LC & 83.14 & 81.83  & 78.38 & 77.10\\
    GAFusion(ours) & LC & \textbf{83.10} & \textbf{81.73}  & \textbf{77.97} & \textbf{76.69}\\
   
    \hline
  \end{tabular}
  \end{adjustbox}
  \caption{Comparison on the Waymo test set. The models in the table are without ensemble or test-time augmentation. }\vspace{-0.2cm}
  \label{tab:waymo_test}
\end{table}
